Linear-Quadratic Zero-Sum Mean-Field Type Games: Optimality Conditions and Policy Optimization

In this paper, zero-sum mean-field type games (ZSMFTG) with linear dynamics and quadratic cost are studied under infinite-horizon discounted utility function. ZSMFTG are a class of games in which two decision makers whose utilities sum to zero, compete to influence a large population of indistinguishable agents. In particular, the case in which the transition and utility functions depend on the state, the action of the controllers, and the mean of the state and the actions, is investigated. The optimality conditions of the game are analysed for both open-loop and closed-loop controls, and explicit expressions for the Nash equilibrium strategies are derived. Moreover, two policy optimization methods that rely on policy gradient are proposed for both model-based and sample-based frameworks. In the model-based case, the gradients are computed exactly using the model, whereas they are estimated using Monte-Carlo simulations in the sample-based case. Numerical experiments are conducted to show the convergence of the utility function as well as the two players' controls.

==> sec_gradient.tex <==


\section{Gradient expression} 
\label{sec2:opt}

\commentJDG{
We now characterize the structure of a Nash equilibrium in terms of linear combinations of the state $x_t$ and conditional mean $\bar x_t$.

To alleviate the notation, let $\tilde A  = A + \bar {A}$, $\tilde Q  = Q + \bar {Q}$, $\tilde B_i  = B_i + \bar {B}_i$, $\tilde R_i  = R_i + \bar {R}_i$, $i=1,2$.  
We recall the notations $\Gamma_i, \Xi_i, \Lambda_i$ introduced in~\eqref{eq:def-GammaXiLambda_i}. 
To investigate the solution of (\ref{eq:prob_for}) and derive the closed-form expressions for the equilibrium controls in terms of the idiosyncratic and mean-field state processes, we introduce the following Riccati equations
\begin{equation}
	\label{eq:main_ARE_P_ZS}
		 \gamma [A^{\top} P + 2Q]\left[ A + \big(B_1 \Gamma_1 + B_2 \Gamma_2\big)  P \right] = P,
	\end{equation}
	and
	\begin{equation}
\label{eq:main_ARE_Pbar_ZS}
	\gamma\bigl[ \tilde A^{\top} \bar{P}+2 \tilde Q\bigr]\left[\tilde A +\big(\tilde B_1\Lambda_1 + \tilde B_2\Lambda_2\big)\bar{P} \right] =\bar{P}.
\end{equation} 

Under suitable conditions and relying on a form of stochastic Pontryagin maximum principle (see \cite{bensoussan2007representation} for the zero-sum case without mean-field interactions and~\cite{CarmonaDelarue_book_I} for the case of mean-field interactions but without zero-sum structure), one can show that the ZSMFTG admits an open-loop Nash equilibrium, say $(\mathrm{\bf u}^*_1, \mathrm{\bf u}^*_2)$. These controls correspond to the open-loop saddle point and can be explicitly written in terms of the solutions $P, \bar P$ of the Riccati equations above as
	\begin{equation}
	\label{eq:MKV-opt-ctrl-formula}
		 u^*_{i,t} = \Gamma_i P(x_t - \bar x_t) + \Lambda_i \bar P \bar x_t, \textrm{ for } i=1,2.
 	\end{equation} 


This relies on a form of stochastic Pontryagin maximum principle for mean-field dynamics. To keep the presentation as concise as possible, we defer the exact statements and the proofs to the appendix, see Propositions~\ref{proposition:Pontryagin_maximum_principle_necessary_condition}, \ref{prop:sufficient_Pontryagin} and Corollary~\ref{corollary:existence_open_loop_Nash} in Appendix~\ref{sec:open-loop-structure}.



According to the above result, it is sufficient to look for  $( K^*_i, L^*_i), i=1,2$ such that
    $$
         u^*_{1,t} = - K^*_1(x^{ \mathrm{\bf u}^*_1, \mathrm{\bf u}^*_2}_t - \bar{x}^{ \mathrm{\bf u}^*_1, \mathrm{\bf u}^*_2}_t) - L^*_1 \bar{x}^{ \mathrm{\bf u}^*_1, \mathrm{\bf u}^*_2}_t,
    $$
    and
    $$
         u^*_{2,t} =  K^*_2(x^{ \mathrm{\bf u}^*_1, \mathrm{\bf u}^*_2}_t - \bar{x}^{\mathrm{\bf u}^*_1, \mathrm{\bf u}^*_2}_t) + L^*_2 \bar{x}^{ \mathrm{\bf u}^*_1, \mathrm{\bf u}^*_2}_t.
    $$



Since optimizing over all possible open-loop controls is infeasible from a numerical perspective (because it is a set of all stochastic processes which does not admit a simple representation), we will focus on closed-loop Nash equilibrium with the above linear structure in the sequel (which allows us to do the optimization over a small number of parameters, namely the coefficients of the linear combination). In fact, it can be shown that looking for closed-loop controls which are linear in $x$ and $\bar x$ leads to the same Nash equilibrium as open-loop controls under suitable conditions (see Appendix~\ref{sec:connect-open-closed}).



\vskip 6pt

}


We henceforth replace problem~\eqref{eq:prob_for} by the following problem, for which optimality conditions have been studied in Section~\ref{sec:closed-loop-structure}.   Each player $i=1,2$ chooses parameter $\theta^*_i = ( K^*_i, L^*_i)$ 
such that
$$
    J(\mathrm{\bf u}^{ \theta^*_1}_1, \mathrm{\bf u}^{\theta^*_2}_2)
    =
    \inf_{\theta_1} \sup_{\theta_2} J(\mathrm{\bf u}^{\theta_1}_1, \mathrm{\bf u}^{\theta_2}_2),
$$
where for $\theta = (\theta_1,\theta_2)$,
$$
    u^{\theta_1,\theta_2}_{i,t} = (-1)^i K_i(x^{\mathrm{\bf u}_1^{\theta_1},\mathrm{\bf u}_2^{\theta_2}}_t 
    - \bar{x}^{\mathrm{\bf u}_1^{\theta_1},\mathrm{\bf u}_2^{\theta_2}}_t) 
    + (-1)^i L_i \bar{x}^{\mathrm{\bf u}_1^{\theta_1},\mathrm{\bf u}_2^{\theta_2}}_t, \qquad i=1,2.
$$

For simplicity, we introduce the following notation
$
    x^{\mathrm{\bf u}_1^{\theta_1},\mathrm{\bf u}_2^{\theta_2}}
    =
    x^{\theta_1,\theta_2},
$
and since we focus on linear controls, we redefine the utility as\todor{already def in closed-loop section?}
$$
    C(\theta_1,\theta_2)
    =
    J(\mathrm{\bf u}^{\theta_1}_1, \mathrm{\bf u}^{\theta_2}_2).
$$
Moreover, we introduce $y^{K_1,K_2}_t = x^{\theta_1,\theta_2}_t - \bar{x}^{\theta_1,\theta_2}_t$ and $z^{L_1,L_2}_t = \bar{x}^{\theta_1,\theta_2}_t$, which is justified by the fact that the dynamics of $\by$ and $\bz$ depend respectively only on $(K_1,K_2)$ and $(L_1,L_2)$. 

Let $P^y_{K_1,K_2}$ be a solution to the linear equation
    \begin{align}
        \label{eq:eq-Py_K1K2}
        P^y_{K_1,K_2}
        &=
        Q + K_1^\top R_1 K_1 - K_2^\top R_2 K_2
        \\
        & \qquad + \gamma (A - B_1 K_1 + B_2 K_2)^\top P^y_{K_1,K_2} (A - B_1 K_1 + B_2 K_2),
        \notag
    \end{align}
and let $P^z_{L_1,L_2}$ be a solution to the linear equation
    \begin{align}
        \label{eq:eq-Pz_L1L2}
        P^z_{L_1,L_2}
        &=
        \tilde Q  + L_1^\top \tilde R_1 L_1 - L_2^\top \tilde R_2 L_2
        \\
        \notag
        & \qquad + \gamma (\tilde A - \tilde B_1 L_1 + \tilde B_2 L_2)^\top P^z_{L_1,L_2} (\tilde A - \tilde B_1 L_1 + \tilde B_2 L_2).
    \end{align}
    
    
\commentJDG{
In order to guarantee that the above equations have solutions, we introduce the notion of stabilizing parameters. 
\begin{definition}
The set of stabilizing parameters is defined as follows:
\begin{align}
    \Theta =
    &\Big\{(K_1,L_1,K_2,L_2) \,:\,
    \gamma \|A - B_1 K_1 + B_2 K_2\|^2 < 1,
    \nonumber \\
    &\quad \gamma \| \tilde A - \tilde B_1 L_1 + \tilde B_2 L_2\|^2 < 1 
    \Big\}.
    \label{eq:Theta_stable_set}
\end{align}
\end{definition}}
We consider the parameter set $\Theta$ introduced in~\eqref{eq:Theta_stable_set}.

\commentJDG{
More details on this closed-loop information structure and the corresponding optimality conditions are provided in Appendix~\ref{sec:closed-loop-structure}.
}


We now prove the following result, which provides an explicit expression for the gradient of the utility function with respect to the control parameters in terms of the solution to the equations~\eqref{eq:eq-Py_K1K2} and~\eqref{eq:eq-Pz_L1L2}.  
\begin{proposition}[Policy gradient expression]
\label{lem:PG_expression}
For any $\theta = (\theta_1,\theta_2) \in \Theta$, we have for $j=1,2$, the gradient
\begin{align}
\label{eq:PG_expression_Kj}
    \nabla_{K_j}C(\theta_1,\theta_2)
    & =
    2 E^{y,j}_{K_1,K_2} \Sigma^y_{K_1,K_2}
\end{align}
where
\begin{align*}
    & 
    \begin{bmatrix}
        E^{y,1}_{K_1,K_2}\\
        E^{y,2}_{K_1,K_2}
    \end{bmatrix}
    = - \gamma  
        \begin{bmatrix} 
        B_1^\top  P^y_{K_1,K_2} A
        \\
      - B_2^\top  P^y_{K_1,K_2} A
        \end{bmatrix}
    +
    \mathbf{R} 
    \begin{bmatrix}
        K_1\\
        K_2
    \end{bmatrix}
\end{align*}
with 
$$
    \mathbf{R} =
    \begin{bmatrix}
        R_1 + \gamma B_1^\top  P^y_{K_1,K_2} B_1 & - \gamma B_1^\top P^y_{K_1,K_2} B_2   
    \\
    - \gamma B_2^\top P^y_{K_1, K_2} B_1 &  - R_2 + \gamma B_2^\top  P^y_{K_1,K_2} B_2 
    \end{bmatrix}
$$
and
$$
    \Sigma^y_{K_1,K_2}
    =\EE\left[ \sum_{t \ge 0} \gamma^t y^{K_1,K_2}_t (y^{K_1,K_2}_t)^\top \right].
$$

Similarly, for $j=1,2$, 
\begin{align*}
    \nabla_{L_j}C(\theta_1,\theta_2)
    & =
    2 E^{z,j}_{L_1,L_2} \Sigma^z_{L_1,L_2}
\end{align*}
where
\begin{align*}
    & 
    \begin{bmatrix}
        E^{z,1}_{L_1,L_2}\\
        E^{z,2}_{L_1,L_2}
    \end{bmatrix}
    = - \gamma  
        \begin{bmatrix} 
        \tilde B_1^\top  P^z_{L_1,L_2} \tilde A
        \\
      - \tilde B_2^\top  P^z_{L_1,L_2} \tilde A
        \end{bmatrix}
    +
    \tilde {\mathbf{R}} 
    \begin{bmatrix}
        L_1\\
        L_2
    \end{bmatrix}
\end{align*}
with 
$$
    \tilde {\mathbf{R}} =
    \begin{bmatrix}
        \tilde R_1 + \gamma \tilde B_1^\top  P^z_{L_1,L_2} \tilde B_1 & - \gamma \tilde B_1^\top P^z_{L_1,L_2} \tilde B_2   
    \\
    - \gamma \tilde B_2^\top P^z_{L_1,L_2} \tilde B_1 &  - \tilde R_2 + \gamma \tilde B_2^\top  P^z_{L_1,L_2} \tilde B_2 
    \end{bmatrix}
$$
and
$$
    \Sigma^z_{L_1,L_2}
    =\EE\left[ \sum_{t \ge 0} \gamma^t z^{L_1,L_2}_t (z^{L_1,L_2}_t)^\top \right].
$$
\end{proposition}
\begin{proof}
    We note that the utility can be split as
    $$
        C(\theta_1,\theta_2)
        =
        \EE_{\tilde y, \tilde z}\Big[
        C_{y}(K_1,K_2, \tilde y)
        +
        C_{z}(L_1,L_2, \tilde z)
        \Big]
    $$
    where
    \begin{align*}
    C_{y}(K_1,K_2, \tilde y) 
    &=
    \EE \sum_{t \ge 0} \gamma^t \Big[
    (y^{L_1,L_2}_t)^{\top} Q y^{K_1,K_2}_t
    \\ 
    &\quad + (u_{1,t}-\bar{u}_{1,t})^{\top} R_{1} (u_{1,t}-\bar{u}_{1,t}) 
    \\
    & \quad - (u_{2,t} - \bar{u}_{2,t})^\top R_{2} (u_{2,t} - \bar{u}_{2,t}) 
    \,|\, y_0 = \tilde y
    \Big]
    \end{align*}
    and
    \begin{align*}
    C_{z}(L_1,L_2, \tilde z) 
    =
    &\EE \sum_{t \ge 0} \gamma^t \Big[
    (z^{L_1,L_2}_t)^{\top} (Q+ \bar Q) z^{L_1,L_2}_t
    \\ 
    &+ \bar{u}^\top_{1,t} (R_{1}+\bar{R}_{1}) \bar{u}_{1,t}
    - \bar{u}^\top_{2,t} (R_{2}+\bar{R}_{2})  \bar{u}_{2,t}
    \,|\, z_0 = \tilde z
    \Big].
    \end{align*}
    Let us consider the first part. We note, using the above definition together with~\eqref{eq:eq-Py_K1K2} and the dynamics satisfied by $y^{K_1,K_2}_t = x^{\theta_1,\theta_2}_t - \bar{x}^{\theta_1,\theta_2}_t$, that
    \begin{align*}
    C_{y}(K_1,K_2, \tilde y) 
    %  
    &= \tilde y^{\top} P^y_{K_1,K_2} \tilde y
    + \frac{\gamma}{1-\gamma} \EE[(\epsilon^1_1)^{\top} P^y_{K_1,K_2} \epsilon^1_1],
    \end{align*}
    from which we deduce that
    $
    \nabla_{\tilde y} C_y(K_1,K_2,\tilde y)
    = 2 P^y_{K_1,K_2} \tilde y.
    $ 
    Moreover,
    \begin{align*}
    C_{y}(K_1,K_2, \tilde y) 
    &=
    \tilde y^\top (Q + K_1^\top R_1 K_1 - K_2^\top R_2 K_2) \tilde y
    \\
    &\quad + \gamma \EE \Big[
    C_{y}\Big(K_1,K_2, (A - B_1 K_1 + B_2 K_2) \tilde y\Big)
    \,|\, y_0 = \tilde y
    \Big].
    \end{align*}
    Using the two above equalities and the chain rule, we obtain (using the fact that $R_1$ is symmetric)
    \begin{align*}
    \nabla_{K_1} C_{y}(K_1,K_2, \tilde y) 
    &=
    2 R_1 K_1 \tilde y \tilde y^\top 
    - 2 \gamma B_1^\top  P^y_{K_1,K_2} (A - B_1 K_1 + B_2 K_2) \tilde y \tilde y^\top
    \\
    &\quad + \gamma \EE \Big[
    \nabla_{K_1} C_{y}\Big(K_1,K_2, \tilde y'\Big)_{\big| \tilde y' = (A - B_1 K_1 + B_2 K_2) \tilde y + \epsilon^1_1}
    \Big].
    \end{align*}
    Using recursion and the equation satisfied by $P^y_{K_1,K_2}$ leads to
    \begin{align*}
    \nabla_{K_1} C_{y}(K_1,K_2, \tilde y) 
    &=
    2 [R_1 K_1  - \gamma B_1^\top  P^y_{K_1,K_2} (A - B_1 K_1 + B_2 K_2)] \times
    \\
    &\quad 
    \left(\tilde y \tilde y^\top 
    + \EE\left[ \sum_{t \ge 1} \gamma^t y^{K_1,K_2}_t (y^{K_1,K_2}_t)^\top \right] \right) .
    \end{align*}
    \todo{omit?}\red{
    Using similar computations, we obtain
    \begin{align*}
    \nabla_{K_2} C_{y}(K_1,K_2, \tilde y) 
    &=
    2 [ - R_2 K_2  + \gamma B_2^\top  P^y_{K_1,K_2} (A - B_1 K_1 + B_2 K_2)] \times
    \\
    &\quad 
    \left(\tilde y \tilde y^\top 
    + \EE\left[ \sum_{t \ge 1} \gamma^t y^{K_1,K_2}_t (y^{K_1,K_2}_t)^\top \right] \right) .
    \end{align*}
    }
    One can proceed similarly for the gradients with respect to $L_1$ and $L_2$.
\end{proof}

